Nonparametric inference of photon energy distribution from indirect measurements

We consider a density estimation problem arising in nuclear physics. Gamma photons are impinging on a semiconductor detector, producing pulses of current. The integral of this pulse is equal to the total amount of charge created by the photon in the detector, which is linearly related to the photon energy. Because the inter-arrival of photons can be shorter than the charge collection time, pulses corresponding to different photons may overlap leading to a phenomenon known as pileup. The distortions on the photon energy spectrum estimate due to pileup become worse when the photon rate increases, making pileup correction techniques a must for high counting rate experiments. In this paper, we present a novel technique to correct pileup, which extends a method introduced in \cite{hall:park:2004} for the estimation of the service time from the busy period in M/G/$\infty$ models. It is based on a novel formula linking the joint distribution of the energy and duration of the cluster of pulses and the distribution of the energy of the photons. We then assess the performance of this estimator by providing an expression of its integrated square error. A Monte-Carlo experiment is presented to illustrate on practical examples the benefits of the pileup correction.

==> Marges.tex <==
% \setlength{\textwidth}{18cm}
% \setlength{\evensidemargin}{0cm}
% \setlength{\oddsidemargin}{0cm}
% \setlength{\textheight}{22.7cm}
% \setlength{\topmargin}{0cm}

% \setlength{\hoffset}{0cm}
% \addtolength{\hoffset}{-1in}
% \addtolength{\hoffset}{1.5cm}

% \setlength{\voffset}{0cm}
% \addtolength{\voffset}{-1in}
% \addtolength{\voffset}{2cm}

% \setlength{\marginparwidth}{0cm}
% \setlength{\marginparsep}{0cm}
% \setlength{\headheight}{16pt}

% CoinCoin !

==> NOTATIONS.tex <==
% Fichier o je mets toutes les notations utilisees pour l'article
% desempilement temps continu via Fourier Method
%
% Thomas Trigano, 12 juillet

% Chemin  pour les graphiques
\graphicspath{{../Figures/Article_juin_2004}}



%%%%%%%%%%%%%%%
% Generalites                          %
%%%%%%%%%%%%%%%


\newcommand{\ttcp}{Type II Counter Problem}
\newcommand{\stdtrip}{(\mathbb{R}_+,{\cal B}(\mathbb{R}_+),\PP)}
\newcommand{\stdtripbidim}{(\mathbb{R}^2_+,{\cal B}(\mathbb{R}^2_+),\PP)}

\newcommand{\ssi}{if and only if }
\newcommand{\iid}{\emph{i.i.d.}}

\newcommand{\funcnorm}[2]{\left\| #1 \right\|_{#2}}

% Pour les mesures de proba associees aux densites...
\newcommand{\probmeas}[1]{\mathrm{P} #1}
\newcommand{\empmeas}{\widehat{\measobs}_{n}}
\newcommand{\emplapobs}{\widehat{\laptot \measobs}_n}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Ensembles Mathématiques                                         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\rme{\mathrm{e}}    % Fonction exponentielle
\def\rmi{\mathrm{i}}    % Imaginaire Pur
\def\nset{\mathbb{N}} % Entiers naturels
\def\zset{\mathbb{Z}} % Entiers relatifs
\def\rset{\mathbb{R}} % Réels
\def\qset{\mathbb{Q}} % Rationnels
\def\cset{\mathbb{C}} % Complexes
\def\PP{\mathbb{P}}             % Espaces de proba
\def\E{\mathbb{E}}              % Espérance d'une var
\def\var{\mathrm{Var}}

\usepackage{ifthen}
\newboolean{pdf}        % Are we using pdftex?
\ifx\pdfoutput\undefined
  \setboolean{pdf}{false}       % Not running pdflatex
  \def\1{\mathbbm{1}}
\else
  \setboolean{pdf}{true}        % Running pdflatex
  \pdfoutput=1
  \def\1{\mathbf{1}}          % mathbbm semble pas marcher avec pdflatex
\fi




\newcommand{\eqsp}{\;}
\newcommand{\eqdef}{\ensuremath{\stackrel{\mathrm{def}}{=}}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Théorèmes et définitions                                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\newtheorem{defi}{Definition}[section]
\newtheorem{hypo}{Assumption}[section]
\newtheorem{ex}{Example}[section]
\newtheorem{propo}{Proposition}[section]
\newtheorem{coro}{Corollary}[section]
\newtheorem{theo}{Theorem}[section]
\newtheorem{lem}{Lemma}[section]
\newtheorem{rema}{Remark}[section]
\newenvironment{demo}[1][]%
{\textbf{#1} }%
{\begin{flushright}$\blacksquare$ \end{flushright}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NOUVELLES DEFINITIONS LIEES A L'ARTICLE                                              %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\densexp}[1]{{\cal E}_{#1}}
\newcommand{\cumenergie}[1]{\bar{E}_{#1}}
\newcommand{\workload}[1]{S_{#1}}

%%%%%%%%%%%%%%%%%%
% Fonctionnelles                               %
%%%%%%%%%%%%%%%%%%

\newcommand{\funk}[2]{\rho(#1,#2)}
\newcommand{\funkname}{\rho}
\newcommand{\funkd}{F_p}
\newcommand{\dcdf}[2]{k(#1,#2)}% VIRER A LA FIN
\newcommand{\dcdm}[2]{\kappa(#1,d#2)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Transformées de Laplace et Fourier  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\laptot}{{\cal L}}
\newcommand{\lapone}{{\cal L}_U}
\newcommand{\laptwo}{{\cal L}_E}
\newcommand{\TF}[1]{#1^*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Variables d'intégration et variables muettes                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\realone}{x}
\newcommand{\realtwo}{y}
\newcommand{\compone}{s}
\newcommand{\comptwo}{p}
\newcommand{\realonemute}{u}
\newcommand{\realtwomute}{v}
\newcommand{\realonemutebis}{w}
\newcommand{\componemute}{\omega}
\newcommand{\comptwomute}{\nu}
\newcommand{\convergeabs}{c}
%\newcommand{\realonemute}{\tau}
%\newcommand{\realtwomute}{\epsilon}

%%%%%%%%%%%%%%%%%%%%%%%%%%
% Noyaux de l'estimateur                                              %
%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\kernel}{K}
\newcommand{\TFkernel}{K^*}
\newcommand{\bandwidth}{h}
\newcommand{\timelimit}{\realone}

%%%%%%%%%%%%%%%%%%%%%%
% Pour la loi ideale                                          %
%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\poissid}{\mathcal{N}}

\newcommand{\densid}{f} % VIRER A LA FIN
\newcommand{\measid}{P}
\newcommand{\Leb}{\mathrm{Leb}}

\newcommand{\funcid}{f_{(U,E)}}

\newcommand{\sampleid}{\{(X_k,Y_k)\}}

\newcommand{\temps}[1]{T_{#1}}
\newcommand{\genericduree}{X}
\newcommand{\genericenergie}{Y}
\newcommand{\duree}[1]{X_{#1}}
\newcommand{\energie}[1]{Y_{#1}}
\newcommand{\couple}[1]{(X_{#1},Y_{#1})}
%\newcommand{\marginal}{f}
\newcommand{\marginal}{m}
\newcommand{\TFmarginal}{m^*}

%%%%%%%%%%%%%%%%%%%%%%%
% Pour la loi observee                                        %
%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\poissobs}{(N_t')_{t\geq 0}}

\newcommand{\densobs}{g}
\newcommand{\measobs}{P'}

\newcommand{\funcobs}{f_{(u,e)}}
\newcommand{\sampleobs}{\{(X'_k, Y'_k)\}}
\newcommand{\genericdureeo}{X'}
\newcommand{\genericenergieo}{Y'}
\newcommand{\tempso}[1]{T'_{#1}}
\newcommand{\dureeo}[1]{X'_{#1}}
\newcommand{\energieo}[1]{Y'_{#1}}
\newcommand{\coupleo}[1]{(X'_{#1},Y'_{#1})}


%%%%%%%%%%%%%%%%%%
% Pour les idles                                 %
%%%%%%%%%%%%%%%%%%

\newcommand{\idle}[1]{Z_{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%
% Dummy variables
%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\auxvar}{\tilde{\lambda}}
\newcommand{\densvar}{\tilde{\densobs}}
\newcommand{\measvar}{\tilde{P}}




\newcommand{\tailexp}{\gamma}
\newcommand{\complem}[1]{#1^{c}}




==> Packages_Eng.tex <==
% Packages
\usepackage{ifthen}
\usepackage{graphicx}
\usepackage{fancyhdr}
\usepackage{fancybox}
\usepackage{lastpage}
\usepackage{multirow}
% Fonts
\usepackage{amsmath}%
\usepackage{amssymb}%
\usepackage{amsfonts}%
\usepackage{bbm}
%\usepackage[T1]{fontenc}
\usepackage{textcomp}
\usepackage{ae}
\usepackage{aecompl}
\usepackage{color}
\normalfont
%Theoremes
\usepackage{amsthm}
%Listes
\usepackage{enumerate}

%Algoritmes.=============================================================
%\usepackage{algorithmic}%
%\usepackage[ruled]{algorithm}%
%\floatname{algorithm}{Algorithme}%
%\renewcommand{\algorithmicrequire}{\textbf{Conditions initiales:}}
%\renewcommand{\algorithmicensure}{\textbf{Ensure:}}
%\renewcommand{\algorithmiccomment}[1]{\{#1\}}
%\renewcommand{\algorithmiccomment}[1]{\emph{#1}}
%\renewcommand{\algorithmicend}{\textbf{fin}}
%\renewcommand{\algorithmicif}{\textbf{si}}
%\renewcommand{\algorithmicthen}{\textbf{alors}}
%\renewcommand{\algorithmicelse}{\textbf{sinon}}
%\renewcommand{\algorithmicelsif}{\algorithmicelse\ \algorithmicif}
%\renewcommand{\algorithmicendif}{\algorithmicend\ \algorithmicif}
%\renewcommand{\algorithmicfor}{\textbf{pour}}
%\renewcommand{\algorithmicforall}{\textbf{pour tout}}
%\renewcommand{\algorithmicdo}{\textbf{faire}}
%\renewcommand{\algorithmicendfor}{\algorithmicend\ \algorithmicfor}
%\renewcommand{\algorithmicwhile}{\textbf{tant que}}
%\renewcommand{\algorithmicendwhile}{\algorithmicend\ \algorithmicwhile}
%\renewcommand{\algorithmicloop}{\textbf{boucle}}
%\renewcommand{\algorithmicendloop}{\algorithmicend\ \algorithmicloop}
%\renewcommand{\algorithmicrepeat}{\textbf{r\'ep\'eter}}
%\renewcommand{\algorithmicuntil}{\textbf{jusqu'\`a}}

